Ada-LEval: Evaluating long-context LLMs with length-adaptable benchmarks

Recently, the large language model (LLM) community has shown increasing interest in enhancing LLMs' capability to handle extremely long documents. As various long-text techniques and model architectures emerge, the precise and detailed evaluation of models' long-text capabilities has become increasingly important. Existing long-text evaluation benchmarks, such as L-Eval and LongBench, construct long-text test sets based on open-source datasets, focusing mainly on QA and summarization tasks. These datasets include test samples of varying lengths (from 2k to 32k+) entangled together, making it challenging to assess model capabilities across different length ranges. Moreover, they do not cover the ultralong settings (100k+ tokens) that the latest LLMs claim to achieve. In this paper, we introduce Ada-LEval, a length-adaptable benchmark for evaluating the long-context understanding of LLMs. Ada-LEval includes two challenging subsets, TSort and BestAnswer, which enable a more reliable evaluation of LLMs' long context capabilities. These benchmarks support intricate manipulation of the length of test cases, and can easily produce text samples up to 128k tokens. We evaluate 4 state-of-the-art closed-source API models and 6 open-source models with Ada-LEval. The evaluation results demonstrate the limitations of current LLMs, especially in ultra-long-context settings. Our code is available at https://github.com/open-compass/Ada-LEval.

==> comparison.tex <==
\section{Comparison with Other Long-Context Benchmarks}

In this section, we compare Ada-LEval with other long-context benchmarks to validate that our benchmarks require much overall text understanding to complete the task than traditional long-context benchmarks.

We regard a task requires models to understand text comprehensively if the performances of models decrease sharply when the text is truncated. 
TSort task meets this requirement since truncating any segment will lead to an incorrect answer.

To exhibit the BestAnswer requires more comprehensive text understanding than traditional QA and summarization tasks, we conduct an experiment on BestAnswer(16k version) and 2 classic long-context datasets, NarrativeQA(LongBench subset, QA task) and GovReport(LongBench subset, summarization task) respectively. 
The metric for NarrativeQA is F1 score and metric for GovReport is Rouge-L. We evaluate the performance of GPT-4-Turbo-1106 on all 3 datasets. Each test case is truncated into 2k, 4k and 8k version as the input. We also provide its full version for comparison.

\begin{table}[h]
    \centering
    \resizebox{1.0\linewidth}{!}{
        \tablestyle{8pt}{1.3}
        \begin{tabular}{c|c|c|c|c|c}
        \shline
        Benchmark & 2k & 4k & 8k & Full & Avg \#tokens \\
        \shline
        BestAnswer & 11.0 & 20.0 & 31.5 & 44.0 & 15646 \\
        NarrativeQA & 24.7 & 25.6 & 29.7 & 33.1 & 10276 \\
        GovReport & 30.7 & 32.4 & 33.6 & 30.9 & 29872 \\
        \shline
        \end{tabular}
    }
    \caption{Results of GPT-4-Turbo on different long-context benchmarks.}
    \label{tab:different_benchmarks}
\end{table}

From the table \ref{tab:different_benchmarks}, the performance of GPT-4-Turbo on BestAnswer decreases more dramatically than NarrativeQA and GovReport when text is truncated. Notably, the performance on GovReport even increases when text is truncated into 4k and 8k. Therefore, our benchmarks require more full-text comprehension than traditional QA and summarization tasks.
